Fast Semantic-Assisted Outlier Removal for Large-scale Point Cloud Registration

With current trends in sensors (cheaper, more volume of data) and applications (increasing affordability for new tasks, new ideas in what 3D data could be useful for); there is corresponding increasing interest in the ability to automatically, reliably, and cheaply, register together individual point clouds. The volume of data to handle, and still elusive need to have the registration occur fully reliably and fully automatically, mean there is a need to innovate further. One largely untapped area of innovation is that of exploiting the {\em semantic information} of the points in question. Points on a tree should match points on a tree, for example, and not points on car. Moreover, such a natural restriction is clearly human-like - a human would generally quickly eliminate candidate regions for matching based on semantics. Employing semantic information is not only efficient but natural. It is also timely - due to the recent advances in semantic classification capabilities. This paper advances this theme by demonstrating that state of the art registration techniques, in particular ones that rely on "preservation of length under rigid motion" as an underlying matching consistency constraint, can be augmented with semantic information. Semantic identity is of course also preserved under rigid-motion, but also under wider motions present in a scene. We demonstrate that not only the potential obstacle of cost of semantic segmentation, and the potential obstacle of the unreliability of semantic segmentation; are both no impediment to achieving both speed and accuracy in fully automatic registration of large scale point clouds.

==> tex/figures/Real_Results.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{tex/figures/Real_AngErr.png}
  \caption{Angular error}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{tex/figures/Real_TrErr.png}
  \caption{Translation error}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{tex/figures/Real_Time.png}
  \caption{Run-time for Optimization}
  \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{tex/figures/Real_TotalTime.png}
  \caption{Total run-time}
  \label{fig:sfig2}
\end{subfigure}
\caption{Performance of the proposed method on the KITTI dataset in comparison to other methods.}
\label{fig:PerformanceKITTI}
\end{figure}

==> tex/figures/Syn_Results.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{tex/figures/Syn_AngErr.png}
  \caption{Angular error}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{tex/figures/Syn_TrErr.png}
  \caption{Translation error}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{tex/figures/Syn_time.png}
  \caption{Run-time for Optimization}
  \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{tex/figures/Syn_Totaltime.png}
  \caption{Total run-time}
  \label{fig:sfig2}
\end{subfigure}
\caption{Performance of the proposed method on semi-synthetic data in comparison to other methods.}
\label{fig:fig}
\end{figure}


==> tex_backup/method.tex <==
\section{Background}
\subsection{Problem Definition}
Before presenting our method, we devote this sub-section to formally define the robust alignment problem. Given two input point clouds $\cM = \{\bm_i \in \bbR^3\}_{i=1}^M$ and $\cN = \{\bn_i \in \bbR^3\}_{i=1}^N$, where $M$ and $N$ represent the number of points in $\cM$ and $\cN$, respectively. Our work addresses large-scale problems in which the number of points in each input point set can be in the ranges of $M,N > 100,000$ points. Following commonly used strategies for robust point cloud alignment, we assume that a set of putative correspondences $\cP$, which can be obtained by several key point extraction techniques (cite some methods), are given as $\cP=\{p_k\}_{k=1}^{D}$, where each correspondence pair $p_k = ( \mathbf{m}_k, \mathbf{n}_{k'} )$ contains $\bm_k \in \cM$ and $\bn_{k'} \in \cN$. Our goal is to estimate the optimal 6-DOF (degrees of freedom) rigid body transformation (i.e., $\bR^* \in SO(3)$ and $\bt^* \in \bbR^3$) that maximizes the following objective function:
\begin{equation}
\label{eq:maxcon_objective}
    (\bR^*, \bt^*) = \arg\max_{\bR, \bt} \sum_{k=1}^{D} \mathbb{I}(\| \mathbf{R}\mathbf{m}_k + \mathbf{t} - \mathbf{n}_{k'} \| \leq \epsilon),
\end{equation}
%our purpose is to utilize semantic information to register them faster and still preserve acceptable accuracy. 
%We first extract initial correspondences $P=\{( \mathbf{m}_i, \mathbf{n}_i )\}_{i=1}^{D}$ between the two point clouds using traditional methods. 
where $\mathbf{R} \in SO(3)$ represents the rotation matrix, $\mathbf{t} \in \mathbb{R}^3$ is the translation vector, and $\|.\|$ denotes the $\ell_2$ Euclidean norm in $\bbR^3$. The indicator function $\mathbb{I}(.)$ returns 1 if its predicate $(.)$ is true and 0 otherwise. Here in~\eqref{eq:maxcon_objective} we employ the commonly used maximum consensus objective function, which has also been used in several other works (cite). The hyper-parameter $\epsilon$ specifies inlier threshold, which can be chosen based on the prior knowledge about the problem.
%is critical to remove outlier influence.

Practically, due to the noisy characteristic of commercial-grade input sensors, and the imperfection of existing feature extraction techniques, $\cP$ may contain a large fraction of outliers. For instance, many problem instances in the KITTI dataset can contain up to $\rho = 90\%$ of outliers (see Table... in our results section), where $\rho$ denotes the outlier ratio. In other words, in order to estimate $\bR^*$ and $\bt^*$, a subset $|\cI^*|$ containing $(1-\rho)D$ inliers must be identified, and vice versa (i.e., if the optimal transformation $(\bR^*, \bt^*)$ is given, $\cI^*$ can easily be obtained). While this problem can be handled effectively by current state-of-the-art algorithms for low $\rho$, a large fraction of outliers may pose a huge challenge to the performance of existing techniques. In this work, we introduce a novel approach to effectively remove outliers in $\cP$ to obtain a subset $\cP' \subset \cP$, where the outlier ratio $\rho'$ of $\cP'$ is much lower than that of the original set $\cP$. Given $\cP'$, the optimal transformation between the two point clouds can be obtained by, e.g., running RANSAC.

To tackle problems with extremely high outlier ratios, our outlier removal approach is motivated by a class of registration methods that attempt to solve point cloud alignment without putative correspondences. In particular, given two sets of points, methods such as (cite) uses pairwise constraints to obtain the optimal set of correspondences by searching for the maximum clique. Such methods make use of geometric information to identify best inlier subset without the need of extracting key points. However, in practice, using all the points as input to such algorithms render it impractical. Therefore, in several works, key points are still used to extract a subset of points as input. 

From the above observation, our work starts by reformulating~\eqref{eq:maxcon_objective} as a maximum clique problem. However, in contrast to existing approaches that solve maximum clique, we introduce a novel integration of semantic information to effectively solve maximum clique. 
To proceed, in the next section, we briefly introduce the Maximum Clique algorithm, which serves as a backbone for our algorithm.
%Typically, large number of outliers exist in $P$.
%If we can find a subset $P' \in P$, where most of correspondences are inliers, it is much easier to estimate 6-DOF transformation. 
\subsection{Maximum Clique Formulation}
\label{sec:max_clique_formulation}
As previously discussed, when the set $\cI^*$ containing the highest number of inliers (set with maximum consensus) is achieved, the optimal transformation $(\bR^*, \bt^*)$ can be obtained using, e.g., SVD. Following (cite), such optimal subset can be found by solving the maximum set of consistent pairs. Specifically, we first define an undirected graph $\cG=(\cV, \cE)$, where each vertex $v_k \in \cV$ corresponds to a pair of correspondences $p_k$ between the two point clouds, i.e., $\cV = \cP $. The set of edges $\cE$ of $\cG$ is defined as 
\begin{equation}
    \label{eq:edge_set_definition}
    \cE = \{ (p_i, p_j) \in \cP \times \cP |  d (p_i, p_j) \le \gamma \}, 
\end{equation}
where the function $d(p_i, p_j)$ specifies the distance between the two correspondence pairs, $p_i = (\bm_i, \bn_{i'}$ and $p_j = (\bm_j, \bn_j')$, which can be expressed as
\begin{equation}
\label{eq:pairwise_distance}
d(p_i, p_j) = | \|\bm_i - \bm_j\| - \|\bn_{i'} - \bn_{j'}\|   |,
\end{equation}
and $\gamma$ is a user-defined threshold. To assist further discussion in later sections, we also define a clique $\cC=(\cV', \cE'), \cV' \subseteq \cV, \cE' \subseteq \cE$ to be a subgraph of $\cG$ in which there exists a connection between any two vertices, i.e., 
\begin{equation}
    \label{eq:clique_edges}
    \cE' = \{v_i, v_j \in \cV | (v_i, v_j) \in \cE \; \forall i,j\}.
\end{equation}
For brevity, we define clique size $|\cC|$ to be the number of vertices $\cC$. A maximum clique $\cC^*$ of $\cG$ is the clique with the maximum number of vertices. For a vertex $v_i \in \cV$, let $\Gamma(v_i)$ be a set that all elements are adjacent to $v_i$, i.e., $\Gamma(v_i) = \{ v_j \in V | (v_i, v_j) \in \cE \}$. We call $|\Gamma(v_i)|$ is the degree of vertex $v_i$. 


Based on the definition as~\eqref{eq:pairwise_distance}, the correspondence pairs $p_i$ and $p_j$ are said to be \emph{consistent} if $d(p_i,p_j) \le \gamma$. The graph $\cG$ defined above is therefore referred to as \emph{consistency graph}. Intuitively, if $p_i$ and $p_j$ both belong to the optimal inlier set $\cI^*$, it is expected that the difference in lengths between the two segments $(\bm_i, \bm_j)$ and $(\bn_{i'}, \bn_{j'})$ must not exceed $\gamma$ (in noise-free settings, $\gamma = 0$).

Given the distance function as defined in~\eqref{eq:pairwise_distance}, the task of optimizing~\eqref{eq:maxcon_objective} boils down to solving for the optimal inlier set $\cI^*$ that contains the maximum number of consistent correspondence pairs, which can be formulated as follows,
\begin{equation}
\label{eq:max_clique}
    \max_{\cI \subseteq \{1,...,D\}} | \cI | \;\;
    \text{s.t.} \,\,\,\, d(p_i, p_j) \leq \gamma \; \forall i, j \in \cI. \\
 %   L(m_i) - L(n_i) = 0 \\
 %   L(m_j) - L(n_j) = 0
%\end{split}   
\end{equation}
Together with the introduction of the consistency graph $\cG$ as discussed above, maximizing~\eqref{eq:max_clique} is equivalent to searching for the maximum clique on $\cG$, which will be discussed in the following section. Interested readers are referred to~\cite{parra19pairwise} and supplementary materials for more details.

%Motivated by \cite{pairwise}, we consider pair of correspondences to approach the problem. Particularly, the distance between two points doesn't change when they move rigidly. In addition, we figure out that the semantic segmentation can be used to remove outliers. We assume the predicted semantic labels of the input point clouds by deep learning network are reliable. The object type of points should be invariant after rigid transformation. 
%To sum up, if two correspondences don’t maintain distance and semantic information, they can’t be both inliers.
%The maximum subset of both pairwise and semantic information consistent correspondences can be the good input for robust registration algorithms (e.g. RANSAC). In general, we attempt to solve:
%where $L(k)$ is the semantic label of a point $k$; and $d((m_i, n_i), (m_j, n_j))$ is the distance between correspondences $(m_i, n_i)$ and $(m_j, n_j)$, which is given by:
%\begin{equation}
%    d((m_i, n_i), (m_j, n_j)) = \|m_i - m_j\|_2 - \|n_i - n_j\|_2
%\end{equation}

%Problem (2) is in a hard computational class (NP-hard problem). Motivated by \cite{parra19pairwise}, we reformulate the problem as maximum clique to efficiently solve this problem. We first formulate an undirected graph G = (V, E) with a set of vertices V and edges E. Each vertex $v_i:=(\mathbf{m}_i, \mathbf{n}_i)$ is the corresponding points that have same semantic information. A pair of vertices $v_i$ and $v_j$ are said to be adjacent, i.e. $(v_i, v_j) \in E$, if they satisfy the pairwise constraints in problem (2).
\subsection{Solving Maximum Clique}
Although the original problem~\eqref{eq:maxcon_objective} can be equivalently formulated as~\eqref{eq:max_clique}, solving~\eqref{eq:max_clique} is still computationally challenging due to the fact that it is NP-hard. To solve~\eqref{eq:max_clique} up to global optimum, therefore, algorithms that are based on branch-and-bound are often used. For instance, Parra~\etal~\cite{parra19pairwise} introduced an efficient algorithm to solve maximum clique by deriving an efficient bounding function. However, such algorithms can only handle input data with modest sizes, while large-scale datasets are still considered impractical. To assist the introduction of our algorithm and for the sake of completeness, in this section, we quickly summarize the general branch-and-bound approach to tackle~\eqref{eq:max_clique}. Our novel modification will be introduced in section 5.

A general strategy for solving maximum clique using branch-and-bound is traversing the graph $\cG$ in a depth-first-search manner. At the beginning  of the algorithm, a node is selected and its adjacent nodes are pushed into a queue for further exploration. During the traversal, the optimal clique size $R^*$ obtained so far is recorded. When visiting a node $v_i$, a bounding function $\tilde{R}(v_i)$ is computed, which provides information about the lower-bound for the maximum clique containing $v_i$ can be achieved. If $\tilde{R}(v_i) + R > R^*$, where $R$ is the current level of the search tree, the search is recursively performed starting from $v_i$. Otherwise, the exploration for $v_i$ is terminated, and the process continues from other nodes in the queue until reaching the optimal solution. More details about branch-and-bound algorithm for maximum clique can be found in~\cite{parra19pairwise}. It is well-known that branch-and-bound has exponential complexity, thus real-time applications rarely employ such techniques, unless the problem size is relatively small.

While the branch-and-bound framework is standard, deriving a tight bounding function $\tilde{R}(v)$ for a particular node is crucial in determining the execution time. Several work, therefore, have proposed different efficient bounding functions for this problem (cite). Most of the work rely on approximate graph-coloring to obtain the lower bound. In addition, other techniques such as ranking the nodes by their degrees, or (Alvaro's technique)~\cite{parra19pairwise} can also be used to speed up the algorithms. However, to the best of our knowledge, most algorithms are still slow for large-scale problems, especially when the graph $\cG$ is dense. 

To address the challenges discussed above, in the following sections, we show how semantic information can be integrated to approximate this problem. In particular, using the provided semantic information containing \NumberOfSemanticClasses different classes, we propose to a theoretically sound approach to decompose the graph into \NumberOfSemanticClasses sub-graphs, and solve maximum clique for the sub-graphs. Notably, we also demonstrate a novel use of information obtained from solved sub-graphs to accelerate the computation of lower-bounding functions during optimizing the remaining sub-graphs. This technique allows us to achieve real-time performance on very large datasets containing an extremely high proportion of outliers.



%A clique in graph G is defined to be a sub-graph where all pairs of vertices are adjacent to each other. Consequently, a maximum clique is a clique with the largest size.


%In this section, we describe some recent global maximum clique algorithms. The following description is mainly included for completeness. 

%\subsection{Branch and Bound Algorithm}
%These will go to supplementary 
% The standard approach for finding maximum clique is based on Branch and Bound. 
% In general, the algorithm discovers set of cliques by applying search tree over the vertices $V$.
% The algorithm begins with the small clique and continues by seeking larger and larger cliques. 
% Precisely, let $R = \{v_1, v_2, ..., v_p\}$ be the current clique, $R_{max}$ be the max clique the algorithm found so far, and $S$ be the set of all candidate vertices that can be added to $R$ to enlarge $R$. In the beginning, $R_{max} := 0$, $R := 0$, $S := V$ (set of all vertices). We choose a vertex $v_i \in S$; then add it in $R$ and compute new set of candidates $S_i = S \cap \Gamma(v_i)$. This procedure is applied until $S_i = 0$.

% When $S_i = 0$, if $R > R_{max}$, $R_{max}$ will be replaced by R. Then, we backtrack and remove $v_i$ from $S$ and $R$. After that, we choose another $v_i$ and continue the same procedure.

% \subsection{Improved algorithms}

% Graph coloring has been employed to make the above branch and bound more efficient. 
% Graph coloring is the process that each vertex $v_i$ is assigned a minimum possible positive integral value $Co[v_i]$, such that no adjacent vertices get same numbers.
% \begin{equation}
%     Co[v_i] \neq Co[v_j] \textnormal{ if } (v_i, v_j) \in E
% \end{equation} 
% where $Co[.]$ is the color or number of vertex. If a graph contains a clique $Q$, at least $|Q|$ colors are needed. As a result, graph coloring can be used to obtain upper bound of $S$ to decide whether expanding $S$ or not. 
% \begin{equation}
%     u_S = |R| + \max\{Co[v_i] \, | \, v_i \in S\}
% \end{equation} 
% where $u_S$ is the upper bound of $S$. If $u_S < |R_{max}|$, there is no chance to find any bigger clique in $S$. Graph coloring is a well known NP-hard problem. In MCQ algorithm \cite{MCQ}, Tomita et al. have employed greedy approximate coloring. To improve MCQ, Parra et al. have proposed a pruning step to help Branch and Bound avoid exploring unnecessary branches during the search.

\section{Method}
\begin{figure}
    \centering
    \includegraphics[width = 340]{tex/figures/mainDiagram1.pdf}
    \caption{Illutrations}
    \label{fig:my_label}
\end{figure}

In this section, we show to make use of the readily available semantic labels to significantly speed up the large-scale registration problems. We first discuss the correspondence pruning using semantic labels. We then introduce the graph decomposition approach, and prove the underlying theory that supports our design choice. The graph decomposition also allows us to derive a novel bounding function that can be quickly evaluated using RANSAC.

%Our technique will be discussed in the following.

\subsection{Correspondence Pruning with Semantic Labels}
A straight-forward utilization of semantic labels in our work is, obviously, to rely on them to prune the set of putative correspondences $\cP$. Specifically, for each 3D points $\bm \in \bbR^3$, let $l(\bm)$ denote the semantic label assigned to $\bm$. If \NumberOfSemanticClasses denotes the number of semantic classes, then $l(\bm) \in \{1, \dots, L\}$. Based on such labelling information, we can obviously prune our set of correspondences $\cP$ by removing correspondences $p_k$ where $l(\bm_k) \ne l(\bn_k')$. Formally, after pruning, we obtain a new set $\cS \subseteq \cP$,
\begin{equation}
    \label{eq:putative_after_prune}
    \cS = \{p_k = (\bm_k, \bn_k') \in \cP | l(\bm_k) = l(\bn_k') \}.
\end{equation}
  
After this pruning procedure, due to the inevitable errors caused by the underlying semantic classifiers, two problems may arise: 
\begin{itemize}
    \item True inliers may be incorrectly removed, and
    \item The set $\cS$ can still contain a large fraction of outliers.
\end{itemize}
For the former problem, our empirical experiments \hl{[we may need to show some graphs here, or refer to some sections in the results that demonstrate this point]} show that the fraction of inliers that are incorrectly removed are insignificant compared to the optimal inlier set $\cI^*$. Moreover, the removed inliers do not cause significant impact to the final estimated transformations compared to ground-truths solutions (See Sec.~\ref{sec:experiments} where we show that the results obtained by our method are competitive to state-of-the-art approaches).
 
 The latter problem, on the other hand, is still a challenging problem. In other words, a robust algorithm still needs to be applied on $\cS$ to remove a large fraction of outliers in $\cS$. One can expect that after pruning, $|\cS| \ll |\cP|$, thus any robust algorithm can easily be applied on this subset $\cS$ to remove outliers. However, this is not the case in many applications. Therefore, executing state-of-the-art robust fitting algorithms on $\cS$ is not easier than the solving original problem. 
 
 In the following section, we show how the provided semantic information can further be utilized to devise a fast algorithm, which can precisely remove outliers in $\cS$.

%These above algorithms have limitations. If the number of edges is large, the run-time of registration algorithms are significantly slow. To solve this problem, we leverage semantic segmentation to improve the run-time. In this section, we propose an approximate but significant faster procedure to find maximum clique.  

\subsection{Semantic Graph Decomposition}

\begin{figure}
    \centering
    \includegraphics[width = 320]{tex/figures/Graph.pdf}
    \caption{Illustrations of Semantic Graph Decomposition. We have 3 semantic classes with 3 different vertex colors (red, yellow, green).
    (a): The original graph with semantic information.
    (b): Maximum cliques of sub-graphs.
    (c): The combined maximum cliques of sub-graphs.
    (d): Maximum clique solved by global optimal algorithm.}
    \label{fig:graph_decomposition}
\end{figure}
%
After executing the semantic pruning procedure as discussed in the previous section to obtain the set $\cS$, let us consider the graph $\cG_S$ build from $\cS$ based on the technique discussed in Section~\ref{sec:max_clique_formulation}. Since the labels assigned to points in each correspondence $p_k =(\bm_k, \bn_{k'}) \in \cS$ are identical, with the abuse of notation, we also use $l(p_k)$ to denote the label associated with points belong to $p_k$, i.e., $l(p_k) = l(\bm_k) = l(\bn_{k'})$. Also, for a graph vertex $v_k \in \cV_S$, we denote by $l(v_k)$ the label of the associated correspondence $p_k$.

Now, define \NumberOfSemanticClasses sub-graphs $\{\cG_i = (\cV_i, \cE_i)\}_{i=1}^L$ extracted from $\cG_S$, where $\cV_i$ comprises correspondences having label $i$, i.e., $\cV_i = \{ v_k \in \cV_S | l(v_k) = i\}$, and $\cE_i = \{ (p_p, p_q) \in \cE_S | l(p_p) = l(p_q) \}$. Observe that by decomposing the original graph $\cG_S$ into \NumberOfSemanticClasses sub-graphs, the total number of vertices remains, while some edges that connect vertices having different labels are temporarily removed. Therefore, the number of edges in each sub-graph can be massively reduced compared to the original graph, i.e., $|\cE_i| \ll |\cE_S| \; \forall i=1,\dots\, L$. \hl{See Figure... for the illustration of graph decomposition}. Moreover, note that based on the sub-graph definitions, in order to obtain the sub-graphs, instead of constructing the original graph $\cG_S$ and perform the decomposition, it is sufficient to just constructing $\cG_i$ based on a subset vertices having label $i$. 



% \begin{prop}
% \label{prop:decomposition}
% Let $\cI^*(\cG)$ be the optimal consensus set obtained after solving~\eqref{eq:max_clique} up to global optimality for the input graph $\cG = (\cV, \cE)$, we have:
% \begin{equation}
%     \cI^*(\cG) \subseteq \bigcup_{i=1}^L \cI^*(\cG_i)
% \end{equation}
% \end{prop}
% \begin{proof}
% Observe that, if $\cI^*(\cG) = \cV$ (i.e., vertices in $\cG$ form a maximum clique), the equality happens. Specifically, if all the vertices in $\cG$ form a maximum clique, there exist connections from each vertex $v_k \in \cV$ to all other vertices. Therefore, any subset of vertices $\cV' \subseteq \cV$ also forms a maximum clique. Consequently, for reach sub-graph $\cG_i$, we have $\cI^*(\cG_i) = \cV_i$. Due to the fact that the total number of vertices are unchanged, we have
% \begin{equation*}
%     \bigcup_{i=1}^L \cI^*(\cG_i) = \bigcup_{i=1}^L \cV_i = \cV = \cI^*(\cG).
% \end{equation*}
% If $\cI^*(\cG) \subset \cV$, define $\cI_i = \{v_k \in \cI^*(\cG) | l(v_k) = i\}$, and it is obvious that $\bigcup_{i=1}^L \cI_i = \cI^*(\cG)$. In addition, it is easy to see that $\cI_i \subseteq \cI^* (\cG_i) \; \forall i = 1\dots L $. Therefore,
% \begin{equation*}
%     \cI^*(\cG) = \bigcup_{i=1}^L \cI_i \subseteq \bigcup_{i=1}^L \cI^* (\cG_i).
% \end{equation*}
% %let $\tilde{\cI} = \cV \setminus \cI(\cG) $ be the set containing the outlying points. For each $v_k \in \tilde{\cI}$, there are two 
% \qed
% \end{proof}
%Proposition~\ref{prop:decomposition} suggests that the task of searching for the optimal inlier set $\cI^*(\cG)$ in the original vertex set of $\cG$ can be achieved by decomposing $\cG$ into $L$ sub-graphs, 
%Proposition~\ref{prop:decomposition} is the main motivation behind our approach. Particularly, instead of  solving~\eqref{eq:max_clique} for the given the input graph $\cG$, which can be difficult since $\cG$ may contain a large number of vertices and edges, we solve $L$ smaller problems, each take $\cG_i$ as input. Finally, the combined solutions from $L$ sub-problems, i.e., $\bigcup_{i=1}^L \cI^* (\cG_i)$,   provides a new correspondence set with a much smaller fraction of outliers.  











%Let maximum clique seek by global algorithm be $MG$ and all vertices with class $l$ in $MG$ be $MG_l$. We propose a novel approach to reduce the run-time of global algorithm.

%For each semantic class $l$, we only build a graph $G_l = (V_l, E_l)$ where $V_l$ are corresponding points with label $l$. We then apply global algorithm to find the maximum clique of class $l$, which is $M_l$.
%We assume that the size maximum clique of each class $M_l$ is always bigger or equal than the size of $MG_l$. Moreover, the elements in $M_l$ may similar to those in $MG_l$. There can be a few different vertices between $M_l$ and $MG_l$. 
%By this way, we find maximum clique of all classes and combine them together. 

\subsection{Initial Lower Bound using Semantic Information}
In this section, we discuss a novel approach to compute a tight lower bound that can effectively speed up the task of solving for $\cI^*(\cG_i)$. 
While classical maximum clique solvers that often rely on variants of graph coloring to compute bounding functions, we make use of the decomposed structure in our problem and utilize the solutions obtained from $\bigcup_{i=1}^{i-1} \cI^*(\cG_i)$ to compute  during the process of solving for $\cI^*(\cG_i)$.



Our new strategy is motivated by the fact that in order to obtain the optimal transformation, only a small subset of correspondences $\hat{\cI} \subset \cI^*$, where $|\hat{\cI}| \ge 3$ is required. Therefore, after obtaining the set $\bigcup_{i=1}^{i-1} \cI^*(\cG_i)$, we aim to seek for this subset. (although may contain outlier --> ransac).   


To speed up our algorithm, we propose an extra step to find initial lower bound on the size of maximum clique. First, we find the maximum clique of $G_l$ with non-moving class $l$. We then run the RANSAC on this maximum clique to achieve transformation parameters $(R_l, t_l)$. After that, we apply this parameters for the next graph $G_{l+1}$ to obtain the approximate number of inliers $I_{l+1}$. The maximum cliques may have outliers
\begin{equation}
    I_l \leq M_l
\end{equation} 
So, the approximate number of inliers can be used for initial lower bound of next class. To make the initial lower bound more efficient, we keep updating $(R_l, t_l)$. After finding maximum clique of $G_{l+1}$, we combine $M_l$ and $M_{l+1}$ together and use RANSAC on it for updating transformation parameters. By this way, $(R_l, t_l)$ gets better and better so that it can discover good initial lower bound.

\subsection{Main Algorithm}
\hl{Pseudo code for the whole system here}
\begin{algorithm}
\caption{Fast Semantic-Assisted Outlier Removal.}
\begin{algorithmic}[1]
\Require A set of putative correspondences $\cP$
\State Initial lower bound $lwb \gets 0$
\State Prune $\cP$ to obtain semantic consistent set $\cS = \{p_k = (\bm_k, \bn_k') \in \cP | l(\bm_k) = l(\bn_k') \}$.
\State Build L sub-graphs $\{\cG_i = (\cV_i, \cE_i)\}_{i=1}^L$
\For{$i = 1, ...,L$}
    \If{($i > 1$)}
        \State $lwb \gets I_{i}$
    \EndIf
    \State Calculate $\cI^*(\cG_i)$ using PMC with $lwb$.
    \If{($|\bigcup_{1}^i\cI^* (\cG_i)| > 3$)}
        \State Estimate ($\bR^*_i$, $\bt^*_i$) using RANSAC on $\bigcup_{1}^i\cI^* (\cG_i)$.
    \EndIf
    \State Calculate initial lower bound for next class $I_{i+1}$
\EndFor
\State Combine solutions from L sub-graphs $\bigcup_{i=1}^L \cI^* (\cG_i)$
\State Estimate ($\bR^*$, $\bt^*$) using robust registration algorithm (e.g. RANSAC) on $\bigcup_{i=1}^L \cI^* (\cG_i)$

\end{algorithmic}
\end{algorithm}



% \begin{prop}
% \label{prop:decomposition}
% Let $\cI^*(\cG)$ be the optimal consensus set obtained after solving~\eqref{eq:max_clique} up to global optimality for the input graph $\cG = (\cV, \cE)$, we have:
% \begin{equation}
%     \cI^*(\cG) \subseteq \bigcup_{i=1}^L \cI^*(\cG_i)
% \end{equation}
% \end{prop}
% \begin{proof}
% Observe that, if $\cI^*(\cG) = \cV$ (i.e., vertices in $\cG$ form a maximum clique), the equality happens. Specifically, if all the vertices in $\cG$ form a maximum clique, there exist connections from each vertex $v_k \in \cV$ to all other vertices. Therefore, any subset of vertices $\cV' \subseteq \cV$ also forms a maximum clique. Consequently, for reach sub-graph $\cG_i$, we have $\cI^*(\cG_i) = \cV_i$. Due to the fact that the total number of vertices are unchanged, we have
% \begin{equation*}
%     \bigcup_{i=1}^L \cI^*(\cG_i) = \bigcup_{i=1}^L \cV_i = \cV = \cI^*(\cG).
% \end{equation*}
% If $\cI^*(\cG) \subset \cV$, define $\cI_i = \{v_k \in \cI^*(\cG) | l(v_k) = i\}$, and it is obvious that $\bigcup_{i=1}^L \cI_i = \cI^*(\cG)$. In addition, it is easy to see that $\cI_i \subseteq \cI^* (\cG_i) \; \forall i = 1\dots L $. Therefore,
% \begin{equation*}
%     \cI^*(\cG) = \bigcup_{i=1}^L \cI_i \subseteq \bigcup_{i=1}^L \cI^* (\cG_i).
% \end{equation*}
% %let $\tilde{\cI} = \cV \setminus \cI(\cG) $ be the set containing the outlying points. For each $v_k \in \tilde{\cI}$, there are two 
% \qed
% \end{proof}
%Proposition~\ref{prop:decomposition} suggests that the task of searching for the optimal inlier set $\cI^*(\cG)$ in the original vertex set of $\cG$ can be achieved by decomposing $\cG$ into $L$ sub-graphs, 
%Proposition~\ref{prop:decomposition} is the main motivation behind our approach. Particularly, instead of  solving~\eqref{eq:max_clique} for the given the input graph $\cG$, which can be difficult since $\cG$ may contain a large number of vertices and edges, we solve $L$ smaller problems, each take $\cG_i$ as input. Finally, the combined solutions from $L$ sub-problems, i.e., $\bigcup_{i=1}^L \cI^* (\cG_i)$,   provides a new correspondence set with a much smaller fraction of outliers.  

%Let maximum clique seek by global algorithm be $MG$ and all vertices with class $l$ in $MG$ be $MG_l$. We propose a novel approach to reduce the run-time of global algorithm.

%For each semantic class $l$, we only build a graph $G_l = (V_l, E_l)$ where $V_l$ are corresponding points with label $l$. We then apply global algorithm to find the maximum clique of class $l$, which is $M_l$.
%We assume that the size maximum clique of each class $M_l$ is always bigger or equal than the size of $MG_l$. Moreover, the elements in $M_l$ may similar to those in $MG_l$. There can be a few different vertices between $M_l$ and $MG_l$. 
%By this way, we find maximum clique of all classes and combine them together. 

